Beyond Correlation: Interpretable Evaluation of Machine Translation Metrics

Machine Translation (MT) evaluation metrics assess translation quality automatically. Recently, researchers have employed MT metrics for various new use cases, such as data filtering and translation re-ranking. However, most MT metrics return assessments as scalar scores that are difficult to interpret, posing a challenge to making informed design choices. Moreover, MT metrics' capabilities have historically been evaluated using correlation with human judgment, which, despite its efficacy, falls short of providing intuitive insights into metric performance, especially in terms of new metric use cases. To address these issues, we introduce an interpretable evaluation framework for MT metrics. Within this framework, we evaluate metrics in two scenarios that serve as proxies for the data filtering and translation re-ranking use cases. Furthermore, by measuring the performance of MT metrics using Precision, Recall, and F-score, we offer clearer insights into their capabilities than correlation with human judgments. Finally, we raise concerns regarding the reliability of manually curated data following the Direct Assessments+Scalar Quality Metrics (DA+SQM) guidelines, reporting a notably low agreement with Multidimensional Quality Metrics (MQM) annotations.

==> tables/dasqm-corr.tex <==
\begin{table}[t]
    \centering
        \begin{tabular}{lrrr}
            \toprule
            & \multicolumn{1}{c}{$\boldsymbol{\tau}$} & \multicolumn{1}{c}{$\boldsymbol{\rho}$} & \multicolumn{1}{c}{\textbf{\acceq}}\\
            \midrule
            \dasqm & $0.11$ & $0.20$ & $0.42$ \\
            \xcomet-\textsc{e} & $0.30$ & $0.42$ & $0.54$ \\
            \comet & $0.25$ & $0.36$ & $0.51$  \\
            \bottomrule
        \end{tabular}
    \caption{Correlations of \dasqm, \xcometens, and \comet, with MQM scores, measured using Pearson $\rho$, Kendall $\tau$ and \acceq accuracy \cite{deutsch-etal-2023-ties}. As recommended by \citet{perrella-etal-2024-guardians}, we used the \textit{Segment Grouping} strategy, meaning that we grouped the translations of the same source segment before computing the correlation values, and then averaged the results across segments. The dataset is the \langpair{zh}{en} split of \wmtth.}
    %Metrics correlations were computed after restricting their assessments to the translations with available DA+SQM annotations.}
    \label{tab:dasqm-corr}
\end{table}

